Generation, estimation, and protection of novel quantum states of spin systems

This thesis deals with the generation, estimation and preservation of novel quantum states of two and three qubits, on an NMR quantum information processor. Using the maximum likelihood ansatz, we have developed a method for state estimation such that the reconstructed density matrix does not have negative eigenvalues and the errors are within the space of valid density operators. Due to interactions with the environment, unwanted changes occur in the system, leading to decoherence. Controlling decoherence is one of the biggest challenges to be overcome to build quantum computers. We have used several experimental strategies to decouple the quantum system from its environment. These strategies are based on how much we know about system-environment interaction and what states we want to preserve. We first consider a case where we are aware of the system state but have no knowledge about its interaction with the environment. We demonstrate the efficacy of the super-Zeno scheme to tackle decoherence in this case. Then we consider a situation where only the subspace is known to which the system state belongs. To address such a situation we used a nested Uhrig dynamical decoupling scheme. Next, we consider situations where we have knowledge of the state of the system as well as its interaction with the environment. In such situations, since the noise model is known, decoupling strategies can be explicitly designed to cancel this noise. Using these decoupling strategies, we can experimentally extend the lifetime of time-invariant discord of two-qubit Bell-diagonal states and are also able to preserve the entanglement of three NMR qubits, to a remarkable extent.

==> Classes/CUEDthesisPSnPDF1.tex <==

%---------------------------------------------------------------
% PhDthesis version 2 style file by Jakob Suckale, 2007
% based on CUEDthesis version 1 by Harish Bhanderi 2002
%---------------------------------------------------------------



%-------------------------- identification ---------------------
%\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{Latex/Classes/PhDthesisPSnPDF}[2007/09/06 v2 PhD thesis class]


%:-------------------------- report or book -----------------------

%If you want to use a Report style document then uncomment the following 3 lines and comment the below 8 book style lines:
%\DeclareOption*{\PassOptionsToClass{\CurrentOption}{report}}
%\ProcessOptions\relax
%%\LoadClass[a4paper]{report}
%\ifx\pdfoutput\undefined
%   \LoadClass[dvips, a4paper]{report}
%\else
%   \LoadClass[pdftex, a4paper]{report}
%\fi

%%Bibliography
%%uncomment next line to change bibliography name to references for Report document class
%\renewcommand{\refname}{References}

%If you want to use a Book style document then uncomment the following 3 lines and comment the above 8 report style lines:
\DeclareOption*{\PassOptionsToClass{\CurrentOption}{book}}
\ProcessOptions\relax
\ifx\pdfoutput\undefined
   \LoadClass[dvips, a4paper]{book}
\else
   \LoadClass[pdftex, a4paper]{book}
\fi


%:-------------------------- packages for fancy things -----------------------

\usepackage{amssymb}
\usepackage{graphics} % for improved inclusion of graphics
%\usepackage{wrapfig} % to include figure with text wrapping around it
\usepackage[margin=10pt,font=small,labelfont=bf]{caption} % for improved layout of figure captions with extra margin, smaller font than text
\usepackage{fancyhdr} % for better header layout
\usepackage{eucal}
\usepackage[english]{babel}
\usepackage[usenames, dvipsnames]{color}
\usepackage[perpage]{footmisc}
\usepackage[sort, numbers, authoryear]{nar}
\usepackage{ifthen}
\usepackage{multicol} % for pages with multiple text columns, e.g. References
\setlength{\columnsep}{20pt} % space between columns; default 10pt quite narrow
\usepackage[nottoc]{tocbibind} % correct page numbers for bib in TOC, nottoc suppresses an entry for TOC itself
%\usepackage{nextpage}

%:-------------------------- Glossary/Abbrev./Symbols -----------------------

\usepackage[intoc]{nomencl} % load nomencl extension; include in TOC
%\nomrefpage % to include page numbers after abbrevations
\renewcommand{\nomname}{Glossary} % rename nomenclature
\renewcommand{\nomlabel}[1]{\textbf{#1}} % make abbreviations bold
\makenomenclature % used to be \makeglossary
\newcommand{\g}{\footnote{For all abbreviations see the glossary on page \pageref{nom}.}} % type "\g" to refer to glossary

% used to be for sorting into categories:
%\renewcommand\nomgroup[1]{%
%  \ifthenelse{\equal{#1}{A}}{%
%   \item[\textbf{Roman Symbols}] }{%             A - Roman
%    \ifthenelse{\equal{#1}{G}}{%
%     \item[\textbf{Greek Symbols}]}{%             G - Greek
%      \ifthenelse{\equal{#1}{R}}{%
%        \item[\textbf{Superscripts}]}{%              R - Superscripts
%          \ifthenelse{\equal{#1}{S}}{%
%           \item[\textbf{Subscripts}]}{{%             S - Subscripts
%	    \ifthenelse{\equal{#1}{X}}{%
%	     \item[\textbf{Other Symbols}]}{{%    X - Other Symbols
%	    \ifthenelse{\equal{#1}{Z}}{%
%	     \item[\textbf{Acronyms}]}%              Z - Acronyms
%              			{{}}}}}}}}}}


%:-------------------------- PDF/PS setup -----------------------

%if you use a macTeX 2008 or later, use the ifpdf package
\usepackage{ifpdf} 

%if you use an older version, uncomment these lines:
%\newif \ifpdf
%    \ifx \pdfoutput \undefined
        % for running latex
%        \pdffalse
%    \else
        % for running pdflatex
%        \pdfoutput = 1    % positive value for a PDF output
                          % otherwise a DVI
%        \pdftrue
%\fi

\ifpdf
%-->
%--> Google.com search "hyperref options"
%--> 
%--> http://www.ai.mit.edu/lab/sysadmin/latex/documentation/latex/hyperref/manual.pdf
%--> http://www.chemie.unibas.ch/~vogtp/LaTeX2PDFLaTeX.pdf 
%--> http://www.uni-giessen.de/partosch/eurotex99/ oberdiek/print/sli4a4col.pdf
%--> http://me.in-berlin.de/~miwie/tex-refs/html/latex-packages.html
%-->
    \usepackage[ pdftex, plainpages = false, pdfpagelabels, 
                 pdfpagelayout = useoutlines,
                 bookmarks,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = false,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref} 

    \DeclareGraphicsExtensions{.png, .jpg, .jpeg, .pdf, .gif} %GIF doesn't work??
    \usepackage[pdftex]{graphicx}
    \pdfcompresslevel=9
    \graphicspath{{0_frontmatter/figures/PNG/}{0_frontmatter/figures/PDF/}{0_frontmatter/figures/}}
\else
    \usepackage[ dvips, 
                 bookmarks,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,
                 linkcolor = black,
                 urlcolor  = black,
                 citecolor = black,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

    \DeclareGraphicsExtensions{.eps, .ps}
    \usepackage{epsfig}
    \usepackage{graphicx}
    \graphicspath{{0_frontmatter/figures/EPS/}{0_frontmatter/figures/}}
\fi


%:-------------------------- page layout -----------------------

%A4 settings
\ifpdf
   \pdfpageheight=297mm
   \pdfpagewidth=210mm
\else
   \setlength{\paperheight}{297mm}
   \setlength{\paperwidth}{210mm}
\fi

\setlength{\hoffset}{0.00cm}
\setlength{\voffset}{0.00cm}

%: Uncomment this secion for two-sided printing
% ------------------------------
\setlength{\oddsidemargin}{1.5cm}
\setlength{\evensidemargin}{0cm}
\setlength{\topmargin}{1mm}
\setlength{\headheight}{1.36cm}
\setlength{\headsep}{1.00cm}
\setlength{\textheight}{20.84cm}
\setlength{\textwidth}{14.5cm}
\setlength{\marginparsep}{1mm}
\setlength{\marginparwidth}{3cm}
\setlength{\footskip}{2.36cm}


%: Uncomment this secion for one-sided printing
% taken from the original file, but with the first two lanes modified
% ------------------------------
%\setlength{\evensidemargin}{1.9cm} % was 1.96cm in original
%\setlength{\oddsidemargin}{-0.001cm} % was -0.54cm in original file
%\setlength{\topmargin}{1mm}
%\setlength{\headheight}{1.36cm}
%\setlength{\headsep}{1.00cm}
%\setlength{\textheight}{20.84cm}
%\setlength{\textwidth}{14.5cm}
%\setlength{\marginparsep}{1mm}
%\setlength{\marginparwidth}{3cm}
%\setlength{\footskip}{2.36cm}


%: section below defines fancy page layout options
% ------------------------------
\pagestyle{fancy}
\renewcommand{\chaptermark}[1]{\markboth{{\thechapter. #1 }}{}}
%\MakeLowercase
\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
\fancyhf{}
\fancyhead[RO]{\bfseries\rightmark}
\fancyhead[LE]{\bfseries\leftmark}
\fancyfoot[C]{\thepage}
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0pt}
\addtolength{\headheight}{0.5pt}
\fancypagestyle{plain}{
  \fancyhead{}
  \renewcommand{\headrulewidth}{0pt}
}





%:-------------------------- title page layout -----------------------

% starts roman page numbering until chapter 1
% important to avoid two pages numbered 1 and 2 which may cause bad links
% bug: cover i + back side ii and then numbering restarts with i; should be iii
\renewcommand{\thepage}{\roman{page}}

\newcommand{\submittedtext}{{A thesis submitted for the degree of}}

% DECLARATIONS
% These macros are used to declare arguments needed for the
% construction of the title page and other preamble.

% The year and term the degree will be officially conferred
\def\degreedate#1{\gdef\@degreedate{#1}}
% The full (unabbreviated) name of the degree
\def\degree#1{\gdef\@degree{#1}}
% The name of your college or department(eg. Trinity, Pembroke, Maths, Physics)
\def\collegeordept#1{\gdef\@collegeordept{#1}}
% The name of your University
\def\university#1{\gdef\@university{#1}}
% Defining the crest
\def\crest#1{\gdef\@crest{#1}}
% Stating the city of birth for title page where needed; uncommented for use
%\def\cityofbirth#1{\gdef\@cityofbirth{#1}}

% These macros define an environment for front matter that is always 
% single column even in a double-column document.

\newenvironment{alwayssingle}{%
       \@restonecolfalse\if@twocolumn\@restonecoltrue\onecolumn
       \else\newpage\fi}
       {\if@restonecol\twocolumn\else\newpage\fi}

%define title page layout
\renewcommand{\maketitle}{%
\begin{alwayssingle}
    \renewcommand{\footnotesize}{\small}
    \renewcommand{\footnoterule}{\relax}
    \thispagestyle{empty}
%  \null\vfill
  \begin{center}
    { \Huge {\bfseries {\@title}} \par}
{\large \vspace*{35mm} {{\@crest} \par} \vspace*{25mm}}
    {{\Large \@author} \par}
%	\vspace*{1ex}
%	{{\@cityofbirth} \par}    
{\large 
	\vspace*{1ex}
    {{\@collegeordept} \par}
	\vspace*{1ex}
    {{\@university} \par}
	\vspace*{25mm}
    {{\submittedtext} \par}
	\vspace*{1ex}
    {\it {\@degree} \par}
	\vspace*{2ex}
    {\@degreedate}
}%end large
  \end{center}
  \null\vfill
\end{alwayssingle}}

% page number for cover back side should have page number blanked


%:-------------------------- front matter layout -----------------------

% DEDICATION
%
% The dedication environment makes sure the dedication gets its
% own page and is set out in verse format.

\newenvironment{dedication}
{\begin{alwayssingle}
  \pagestyle{empty}
  \begin{center}
  \vspace*{1.5cm}
  {\LARGE }
  \end{center}
  \vspace{0.5cm}
  \begin{quote} \begin{center}}
{\end{center} \end{quote} \end{alwayssingle}}


% ACKNOWLEDGEMENTS
%
% The acknowledgements environment puts a large, bold, centered 
% "Acknowledgements" label at the top of the page. The acknowledgements
% themselves appear in a quote environment, i.e. tabbed in at both sides, and
% on its own page.

\newenvironment{acknowledgements}
{\pagestyle{empty}
\begin{alwayssingle}
\begin{center}
\vspace*{1.5cm}
{\Large \bfseries Acknowledgements}
\end{center}
\vspace{0.5cm}
\begin{quote}}
{\end{quote}\end{alwayssingle}}

% The acknowledgementslong environment puts a large, bold, centered 
% "Acknowledgements" label at the top of the page. The acknowledgement itself 
% does not appears in a quote environment so you can get more in.

\newenvironment{acknowledgementslong}
{\pagestyle{empty}
\begin{alwayssingle}
\begin{center}
\vspace*{1.5cm}
{\Large \bfseries Acknowledgements}
\end{center}
\vspace{0.5cm}\begin{quote}}
{\end{quote}\end{alwayssingle}}

%ABSTRACT
%
%The abstract environment puts a large, bold, centered "Abstract" label at
%the top of the page. The abstract itself appears in a quote environment,
%i.e. tabbed in at both sides, and on its own page.

\newenvironment{abstracts} {
\pagestyle{empty}
\begin{alwayssingle} 
  \begin{center}
  \vspace*{1.5cm}
  {\Large \bfseries  Abstract}
  \end{center}
  \vspace{0.5cm}
   \begin{quote}}
{\end{quote}\end{alwayssingle}}

%The abstractlong environment puts a large, bold, centered "Abstract" label at
%the top of the page. The abstract itself does not appears in a quote
%environment so you can get more in.

\newenvironment{abstractslong} {\pagestyle{empty}
\begin{alwayssingle} 
  \begin{center}
  \vspace*{1.5cm}
  {\Large \bfseries  Abstract}
  \end{center}
  \vspace{0.5cm} \begin{quote}}
{\end{quote}\end{alwayssingle}}

%The abstractseparate environment is for running of a page with the abstract
%on including title and author etc as required to be handed in separately

\newenvironment{abstractseparate} {\begin{alwayssingle} \pagestyle{empty}
  \vspace*{-1in}
 \begin{center}
    { \Large {\bfseries {\@title}} \par}
    {{\large \vspace*{1ex} \@author} \par}
{\large \vspace*{1ex}
    {{\@collegeordept} \par}
    {{\@university} \par}
\vspace*{1ex}
    {{\it \submittedtext} \par}
    {\it {\@degree} \par}
\vspace*{2ex}
    {\@degreedate}}
  \end{center} \begin{quote}}
{  \end{quote} \end{alwayssingle}}

%Statement of originality if required

\newenvironment{declaration} {\begin{alwayssingle} \pagestyle{empty}
  \begin{center}
  \vspace*{1.5cm}
  {\Large \bfseries  Declaration}
  \end{center}
  \vspace{0.5cm}
   \begin{quote}}
{\end{quote}\end{alwayssingle}}


%:-------------------------- page numbers: roman+arabic -----------------------

% ROMANPAGES
%
% The romanpages environment set the page numbering to lowercase roman one
% for the contents and figures lists. It also resets
% page-numbering for the remainder of the dissertation (arabic, starting at 1).

%\newenvironment{romanpages}
%{
%	\setcounter{page}{1}
%	\renewcommand{\thepage}{\roman{page}}
%} % close romanpage env't
 
{\newpage\renewcommand{\thepage}{\arabic{page}}\setcounter{page}{1}}



==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 

